Robustness Evaluation of Entity Disambiguation Using Prior Probes:the Case of Entity Overshadowing

Entity disambiguation (ED) is the last step of entity linking (EL), when candidate entities are reranked according to the context they appear in. All datasets for training and evaluating models for EL consist of convenience samples, such as news articles and tweets, that propagate the prior probability bias of the entity distribution towards more frequently occurring entities. It was previously shown that the performance of the EL systems on such datasets is overestimated since it is possible to obtain higher accuracy scores by merely learning the prior. To provide a more adequate evaluation benchmark, we introduce the ShadowLink dataset, which includes 16K short text snippets annotated with entity mentions. We evaluate and report the performance of popular EL systems on the ShadowLink benchmark. The results show a considerable difference in accuracy between more and less common entities for all of the EL systems under evaluation, demonstrating the effects of prior probability bias and entity overshadowing.

==> scrap.tex <==
% we compare the predictions on the \textit{Top} and \textit{Shadow} subsets with the predictions of the same model on the \textit{Neutral} subset.
% Thus, $pred=prior$ denotes that the prediction is the same as the "default" prediction of the model for the same entity mention. 

% \begin{figure}[h!]
%      \vspace*{-0.9em}
%      \begin{subfigure}[b]{\columnwidth}
%         \includegraphics[width=\textwidth]{rel_results_shadowlink.png}
%         %  \caption{REL}
%          \label{fig:rel_shadowlink}
%      \end{subfigure}
%     %  \hfill
%     %  \hspace{0.25cm}
%      \vspace*{-0.9em}
%     \begin{subfigure}[b]{\columnwidth}
%         \includegraphics[width=\textwidth]{tagme_results_shadowlink.png}
%         %  \caption{TagMe}
%          \label{fig:tagme_shadowlink}
%      \end{subfigure}
%          \vspace*{-0.9em}
%     \begin{subfigure}[b]{\columnwidth}
%         \includegraphics[width=\textwidth]{wat_results_shadowlink.png}
%         %  \caption{WAT}
%          \label{fig:wat_shadowlink}
%      \end{subfigure}
%      \caption{Results on the ShadowLink dataset \sv{what results? what is the metrics? what is x and y?}}
%     \label{fig:results_barplot}
% \end{figure} 

% The results of evaluating priors (?) are presented in Table~\ref{tbl:big-results-table}.


\begin{table*}[h!]
\centering
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{c}{\textbf{Aspect}} & \multicolumn{1}{c}{\textbf{ShadowLink}} & \multicolumn{1}{c}{\textbf{WikiDisamb30}} & \multicolumn{1}{c}{\textbf{KORE50}} & \multicolumn{1}{c}{\textbf{Guo et al.}} \\
 \hline
\begin{tabular}[c]{@{}l@{}}source \end{tabular} & Web & Wikipedia & \begin{tabular}[c]{@{}l@{}}manual \end{tabular} & \begin{tabular}[c]{@{}l@{}} Web \end{tabular} \\
% \begin{tabular}[c]{@{}l@{}}designed to evaluate\\  prior biases?\end{tabular} & yes & no & no & yes \\
long-tail entities & \checkmark & - & \checkmark & - \\
publicly available & \checkmark & \checkmark & \checkmark & - \\
\begin{tabular}[c]{@{}l@{}} \# mentions\end{tabular} & \begin{tabular}[c]{@{}l@{}} 2.7K \\ %(904*3, not counting neutral)% 
\end{tabular} & 1.4M & 148 & - \\
\hline
\end{tabular}
% }
\caption{\label{tbl:datasets} ShadowLink in comparison with other datasets for the ED task.}
\end{table*}


%


% We show that the impact of such biases can be measured by comparing the predictions of a system on a neutral context with the predictions on the same entity mention in a meaningful context.

% The difference in accuracy on top and shadow entities indicates that EL predictions are biased towards more common entities.
% We used a graph-based measure of commonness (the number of links pointing to the entity page), and it appears to be a good predictor of the EL task complexity on the ambiguous entities.
% : less common entities are harder to link compared to the more common ones.
% However, commonness alone is not predictive enough: it appears that ambiguity is more important (see RQ4)

% At the same time, we show that human annotators do not rely on the entity commonness and are able to disambiguate between the two sets equally well.
% are better and rely less on bias} 


==> scrap_5_results.tex <==
\subsection{Benchmark Results}
% \section{Benchmark Experiments}
% \todo{briefly describe the content as a whole what are we going to present here, repeat and answer the RQs}

This section presents the results of our experiments  and summarizes the answers to the research questions introduced in Section~\ref{sec:intro}.
% this study.
% : the evaluation of baseline models performance on \OurDataset, the results of manual evaluation, and the answers to the research questions addressed in this study. 
% \subsection{Benchmark evaluation}
% \todo{answers to RQs: what did we find out wrt each of our RQs}

\textbf{RQ1:} Are EL predictions biased and how can we measure it?\\

EL predictions appear to be influenced by prior biases. The impact of such biases can be measured by comparing the predictions of a system on a neutral context with the predictions on the same entity mention in a meaningful context.


\textbf{RQ2:} Are EL predictions biased towards more common entities? How can we measure commonness and is it predictive of the EL performance?\\

The difference in accuracy on top and shadow entities indicates that EL predictions are biased towards more common entities. We used a graph-based measure of commonness (the number of links pointing to the entity page), and it appears to be a predictor of EL task complexity: less common entities are harder to link compared to more common ones. However, commonness alone is not predictive enough: it appears that ambiguity is more important (see RQ4)

\textbf{RQ3:} How well can the existing EL systems recognise overshadowed entities?\\

All of the EL systems considered in our study have significantly lower accuracy on overshadowed entities compared to top entities. [human annotators are better and rely less on bias]. 

\textbf{RQ4:} How does the performance on overshadowed entities compare to other long-tail but unambiguous entities? \\

The EL systems achieve significantly higher accuracy on unambiguous long-tail entities (TailLink) compared to both top and overshadowed entities in ShadowLink. This indicates that ambiguity could be a stronger predictor of EL task complexity than commonness.

% \todo{RQ4}
% \textbf{Overall accurracy.}
Table~\ref{tbl:res-all} compares the systems' accuracy across the ShadowLink subsets.

\begin{table}[]
\centering
\begin{tabular}{lccc}
\hline
    \textbf{Baseline}           & \textbf{Top} & \textbf{Shadow} & \textbf{Tail} \\
\hline   
REL   & 53.65       & 20.69          & 91.37  \\
TagMe & 52.43 &  28.10   & 76.44        \\
WAT   & 48.45       & 25.11          & 60.29       \\
\hline
\end{tabular}
\caption{\label{tbl:res-all} \% of the correctly linked entities for the ShadowLink subsets.}
\end{table}

All systems show the highest accuracy results on the \textit{Tail} subset.
\sv{what does that show?}

REL outperforms TagMe and WAT on the Top and Tail subsets but scores the lowest on the Shadow, which suggests that ... 
\sv{how can we explain this dependency?}

% The results on the ShadowLink, however, are significantly lower, which indicates that high ambiguity is a bigger obstacle for ED than low commonness.
Overshadowed entities (the Shadow subset) are the most challenging for all the systems, with the maximum accuracy of 28.1\% achieved by TagMe.
\todo{These findings are consistent with \citeauthor{ilievski-etal-2018-systematic}~(\citeyear{ilievski-etal-2018-systematic}), who suggested that the combination of ambiguity and commonness should be a good predictor of complexity of the EL task.}

% \textbf{Quality assurance for ShadowLink.}
\todo{To ensure that the results are consistent with the results.. we evaluate on the same subset that was used for manual evaluation.}

% are accurate, we selected a smaller sample from the manual evaluation dataset, choosing only from the examples considered clear by both annotators.
The sample included 38 top and 41 shadow entities. We then evaluated the baseline models on this sample to check whether the results are consistent with the results on the whole ShadowLink dataset. Table~\ref{tab:sample_results} shows the resulting accuracy:

\todo{check why the difference is large between the two tables: eg tagme shadow}

\begin{table}[]
\centering
\begin{tabular}{lcc}
\hline
  Baseline   & \textbf{Top} & \textbf{Shadow} \\
\hline
REL   & 55.26              & 19.51                 \\
TagMe & 55.26              & 48.78                 \\
WAT   & 47.37              & 19.51          \\  
\hline
Human   & \sv{x}              & \sv{93.48}          \\   
\hline
\end{tabular}
\caption{\label{tab:sample_results} Benchmarking results on the manually contolled sample}
\end{table}
%
The results for REL and WAT on the smaller subset are consistent with the overall results presented in Table~\ref{tbl:res-all}. For TagMe, there is a noticeable increase in accuracy on the shadow sample; however, the accuracy on the shadow entities for all systems remains significantly lower than the accuracy on the top ones, proving that shadow entities are indeed harder to disambiguate.

\todo{comment on the diff with human performance}

%
\textbf{Impact of priors.}
% Figure~\ref{fig:results_barplot} shows detailed evaluation results for ShadowLink.
To evaluate the impact of priors, ...
% we compare the predictions on the \textit{Top} and \textit{Shadow} subsets with the predictions of the same model on the \textit{Neutral} subset.
% Thus, $pred=prior$ denotes that the prediction is the same as the "default" prediction of the model for the same entity mention. 

\begin{figure}[h!]
     \vspace*{-0.9em}
     \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{rel_results_shadowlink.png}
        %  \caption{REL}
         \label{fig:rel_shadowlink}
     \end{subfigure}
    %  \hfill
    %  \hspace{0.25cm}
     \vspace*{-0.9em}
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{tagme_results_shadowlink.png}
        %  \caption{TagMe}
         \label{fig:tagme_shadowlink}
     \end{subfigure}
         \vspace*{-0.9em}
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{wat_results_shadowlink.png}
        %  \caption{WAT}
         \label{fig:wat_shadowlink}
     \end{subfigure}
     \caption{Results on the ShadowLink dataset \sv{what results? what is the metrics? what is x and y?}}
    \label{fig:results_barplot}
\end{figure} 

\todo{For all systems, the majority of correct answers on the \textit{Top} dataset coincides with the prior predictions obtained for the same entity mention in neutral context.
On the \textit{Shadow} subset we can see the opposite trend: most of the wrong predictions are the same as priors, and most of the correct ones are different.
This indicates that the impact of commonness outweighs the impact of relatedness, preventing the systems from finding the correct answer despite the presence of context information.}

\todo{We also analyse the impact of priors by considering two cases: overshadowing itself, when the prediction for an entity mention is the same for both \textit{top} and \textit{shadow} examples, and prior bias, when the default prediction of the system does not change at all when presented with different context.
Figure~\ref{fig:prior_bias} shows the number of these cases for each system.}


\begin{figure}[h!]
    % \centering
    \includegraphics[width=\columnwidth]{bias_barplot.png}
    \caption{Overshadowing and prior bias on ShadowLink. \sv{what results? what is the metrics? what is x and y?}}
    \label{fig:prior_bias}
\end{figure}

\todo{Among the three systems, REL turns out to be the most prone to overshadowing and the least likely to change its predictions based on context.
This explains its accuracy drop on ShadowLink compared to the unambiguous TailLink dataset.
TagMe and WAT, on the other hand, appear to be more sensitive to the impact of local context, which allows them to achieve better results on \textit{shadow} entities.}

\todo{big results table}
\upd{done}

\begin{table}*[h!]
\begin{tabular}{llllll|lllll}
 & \multicolumn{5}{l|}{Top} & \multicolumn{5}{c|}{Shadow} \\
 & \multicolumn{2}{l}{pred = prior} & \multicolumn{2}{l}{pred != prior} & \multirow{2}{*}{NIL} & \multicolumn{2}{l|}{pred = prior} & \multicolumn{2}{l}{pred != prior} & \multirow{2}{*}{NIL} \\
 & correct & wrong & correct & wrong &  & correct & wrong & correct & wrong &  \\ \cline{2-11} 
REL & .3230 & .2478 & .2135 & .2102 & .0055 & .0774 & .5088 & .1294 & .2788 & .0055 \\
TagMe & .2843 & .1516 & .2400 & .1726 & .1515 & .0531 & .2920 & .2279 & .2688 & .1582 \\
WAT & .3208 & .1173 & .1637 & .1239 & .2743 & .0420 & .3175 & .2091 & .1560 & .2754
\end{tabular}
\caption{\label{tbl:big-results-table} Results with priors on ShadowLink}
\end{table}

% \todo{the results have changed tonight (30.01), will be updated soon}
% \begin{table}[h] 
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{@{}clllll@{}}
%     \multicolumn{1}{l}{}                  &               & \textbf{REL} & \textbf{TagME} & \textbf{WAT} \\ %& \textbf{End2End} \\
%     \multirow{2}{*}{\textbf{correct, \%}} & pred = prior  & 31.31        &    29.20           &   28.65    \\% &  6.69   \\
%                                           & pred != prior & 22.35        &    23.00      & 19.80 \\ %& 0? \\
%     \multirow{2}{*}{\textbf{wrong, \%}}   & pred = prior  & 28.76        &    16.70           &   11.28     \\  % & 3.41   \\
%                                           & pred != prior & 17.59        &    31.08            & 40.27        % &  89.9 (NIL)  
%     \end{tabular}
% }
% \caption{\label{res-top} Benchmarking results on the top dataset}
% \end{table}

% \sv{what detailed results? what does this table show? what are the numbers? what is the metrics used?}

% \begin{table}[h]
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{@{}clllll@{}}
    
%     \multicolumn{1}{l}{}                  &               & \textbf{REL} & \textbf{TagME} & \textbf{WAT} &  \\ % \textbf{End2End} \\
%     \multirow{2}{*}{\textbf{correct, \%}} & pred = prior  &  9.07        &    8.41      & 6.31  \\ % &\\
%                                           & pred != prior & 11.62        &   19.58  &  18.81 
%                                           \\ %& 1.28 \\
%     \multirow{2}{*}{\textbf{wrong, \%}}   & pred = prior  & 52.54        &  31.75    & 28.88 \\ 
%     % & ..              \\
%                                           & pred != prior & 24.78        &   40.27  & 47.01    %  & ..           
%     \end{tabular}
% }
% \caption{\label{res-shadow} Benchmarking results on the overshadowed dataset}
% \end{table}



% \begin{table}[h]
% \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lll}
%                   & \textbf{pred(top) = pred(shadow), \%} & \textbf{pr(top) =  pr(shadow) = pr(neutral), \%} \\
%     \textbf{REL}   & 57.08  & 46.35  \\
%     \textbf{TagME} & 29.54    & 23.34  \\
%     \textbf{WAT}   & 23.67     &  17.92     \\
%     % \textbf{End2End}   &          &    
%     \end{tabular}
% }
% \caption{\label{overshadowing} Percentage of cases where overshadowing occurs}
% \end{table}


% [poor results on end2end because it only works for mentions it has seen before: Most of the wrong predictions made by the End2End algorithm are due to the system not recognising the mentions that have not occured in its training data: for such mentions, the algorithm outputs an empty answer (89.9\% on the top dataset and 91.47\% on the overshadowed dataset). However, when the algorithm does recognise the mention, ]



%
% \subsection{Discussion}
% \todo{distribute the question/answers along with the results presentations}
%
% Analysing the results gives the following answers to the research questions considered in this paper: \\


==> scrap_rq3.tex <==
\textbf{RQ3:} Does human performance differ for overshadowed entities?
% \textbf{Quality assurance for ShadowLink.}
% To ensure that the results are consistent we evaluate on the same subset that was used for manual evaluation.
% are accurate, we selected a smaller sample from the manual evaluation dataset, choosing only from the examples considered clear by both annotators.
% The sample included 38 top and 41 shadow entities.
We also evaluate our baselines on the sample used for manual evaluation to check whether the results are consistent with the results obtained on the full ShadowLink dataset. Table~\ref{tab:sample_results} shows the accuracy on this smaller sample (37 top- and 40 shadow-entities).
% \todo{check why the difference is large between the two tables: eg tagme shadow}
\begin{table}[]
\centering
\begin{tabular}{lcc}
\hline
  \textbf{Baseline}   & \textbf{Top} & \textbf{Shadow} \\
\hline
TagMe & 54.05              & 47.50          \\
WAT   & 48.65              & 37.50          \\  
REL   & 56.76              & 22.50          \\
\hline
Human   & 98.65              & 98.78          \\   
\hline
\end{tabular}
\caption{\label{tab:sample_results} Benchmarking results on the manually contolled sample.}
\end{table}
%
The results for REL on the smaller subset are consistent with the overall results presented in Table~\ref{tbl:res-all}. For TagMe and WAT, there is a noticeable increase in accuracy on the shadow sample; however, the accuracy on the shadow entities for all systems remains lower than the accuracy on the top-entities, proving that shadow entities are indeed harder to disambiguate.
% \todo{TagMe is not much lower}
All of the EL systems considered in our study have much lower accuracy than human annotators showing a large performance gap for the automated approaches.
% \todo{do we have separate results for how many errors are due to the incorrect mention detection?}
% \upd{no, but it would only be a problem for TagMe - REL and WAT support the ED-only setting}
Also, the difference in accuracy for Top and Shadow is large for the baseline results, while the human annotators are able to disambiguate between the two subsets equally well.
% \todo{comment on the diff with human performance}
% The results also show that the difference in accuracy for Top and Shadow entities in manual disambiguation is much smaller than in the systems' results.
